Generation Of A Complete Set Of Properties

One of the problems of formal verification is that it is not functionally complete due the incompleteness of specifications. An implementation meeting an incomplete specification may still have a lot of bugs. In testing, this issue is addressed by replacing functional completeness with $\mathit{structural}$ one. The latter is achieved by generating a set of tests probing every piece of a design implementation. We show that a similar approach can be used in formal verification. The idea here is to generate a property of the implementation at hand that is not implied by the specification. Finding such a property means that the specification is not complete. If this is an $\mathit{unwanted}$ property, the implementation is buggy. Otherwise, a new specification property needs to be added. Generation of implementation properties related to different parts of the design followed by adding new specification properties produces a $\mathit{structurally}$-$\mathit{complete\:specification}$. Implementation properties are built by $\mathit{partial\: quantifier\:elimination}$, a technique where only a part of the formula is taken out of the scope of quantifiers. An implementation property is generated by applying partial quantifier elimination to a formula defining the "truth table" of the implementation. We show how our approach works on specifications of combinational and sequential circuits.

==> a0ny_prop.tex <==
\section{Any Property Can Be Generated By PQE}
\label{app:any_prop}
Let $F(X,Y,Z)$ be a formula specifying a combinational circuit
$N(X,Y,Z)$.  In this appendix, we prove that by combining clause
splitting with PQE one can generate any property of $N$. The procedure
used in this proof is not very realistic because it requires an
exponential blow-up of the formula. Nevertheless, our result has some
practical meaning, which is twofold. First, clause splitting
significantly \ti{extends} the set of properties that can be generated
by PQE. Second, there is a set of properties \ti{natural} to $N$ that
can be \ti{efficiently} produced by clause splitting and PQE. Those
are the properties that can be generated without an exorbitant amount
of clause splitting.


Let $Q(V)$ be a property of $N$ where $V \subseteq (X \cup Z)$. So
$F \imp Q$.  Let us show that $Q$ can be obtained by applying PQE to
formula \prob{W}{G} where $W = \V{G} \setminus V$ and $G$ is obtained
from $F$ by clause splitting. (So $\V{G} = \V{F} = X \cup Y \cup Z$.)
Formula $G$ is obtained by splitting the clauses of $F$ on variables
of $V$ that is different from that of Definition~\ref{def:cls_split}.
Namely, every clause $C \in F$ is replaced with $2^{|V|}$ clauses
$C \vee \cls{B}{v}$ where \pnt{v} is an assignment to $V$
and \cls{B}{v} is the longest clause falsified by \pnt{v}. Note that
if $C$ and \cls{B}{v} have opposite literals of a variable $w \in
(\V{C} \cap V)$ then the clause $C \vee \cls{B}{v}$ is tautologous and
can be removed from the formula $G$. Denote by $G_1$ (respectively
$G_2$) the clauses $C \vee \cls{B}{v}$ where \pnt{v} falsifies
(respectively satisfies) the property $Q$.
%
\begin{proposition}
\label{prop:any_prop}
The property $Q$ above is a solution to the PQE problem of taking
$G_1$ out of the scope of quantifiers in \prob{W}{G_1 \wedge G_2}.
That is $\prob{W}{G_1 \wedge G_2} \equiv Q \wedge \prob{W}{G_2}$.
\end{proposition}
%
\begin{proof}
One needs to show that for every assignment \pnt{v} to $V$, formulas
$G_1 \wedge G_2$ and $Q \wedge G_2$ are equisatisfiable in
subspace \pnt{v}. Consider the following two cases.
\begin{itemize}
\item $Q(\pnt{v}) = 0$. By construction, $G_1 \wedge G_2$ is logically equivalent to $F$.
The fact that $F \imp Q$ entails that $G_1 \wedge G_2$ is
unsatisfiable in subspace
\pnt{v}. So both $G_1 \wedge G_2$ and $Q \wedge G_2$ are unsatisfiable in
subspace \pnt{v}.
\item $Q(\pnt{v}) = 1$. By construction, every clause $C \wedge \Cls{B}{v}$ of $G_1$
is satisfied by \pnt{v} (because $\pnt{v} \neq \Pnt{v}$). So
$G_1 \wedge G_2$ and $Q \wedge G_2$ are logically equivalent
in subspace \pnt{v}.
\end{itemize}
\end{proof}


==> c2ompl_set_of_incons_props.tex <==
%\section{Structually Complete Set Of Properties (combinational circuits)}
%\section{Structurally Complete Set Of Tests}
\section{Complete Set Of Inconsistent Properties}
\input{s2tr_comp_incons_props.fig}
%




==> f2ootnote.tex <==
\label{ftn:circ_to_form}
A formula $F(X,Y,Z)$ \ti{specifies} the circuit $N(X,Y,Z)$, if every
assignment satisfying $F$ corresponds to a consistent assignment to
the variables of $N$ and vice versa. An assignment to the variables of
$N$ is called consistent if it is consistent for every gate $G$ of $N$
i.e.  the value assigned to the output variable of $G$ is implied by
the values assigned to the input variables of $G$.


==> i2ntegr_tests_by_pqe.tex <==
\section{Integrity Tests By PQE}


==> m1ain_loop_seq.fig.tex <==
%
% PPT_sc procedure (Structurally Complete set of properties, Sequential Case)
%
\setlength{\intextsep}{4pt}
\setlength{\textfloatsep}{10pt}
%% \begin{wrapfigure}{l}{1.6in}
\begin{figure}
%\begin{center}
\centering
\small
%\normalsize
%\vspace{5pt}
\parbox{0cm}{\begin{tabbing}
%\begin{tabbing}
aaa\=b\=c\= d\= \kill
$\ppts(T,I,n)$\{\\
\tb{\scriptsize{1}}\> $\mi{Cls}:=T$    \\
\tb{\scriptsize{2}}\> $\mi{Props} := \emptyset$ \\
\tb{\scriptsize{3}}\> $\mi{Trcs} := \emptyset$ \\
\tb{\scriptsize{4}}\> while $(\mi{Cls} \neq \emptyset)$ \{ \\
\tb{\scriptsize{5}}\Tt  $C := \mi{PickCls}(Cls)$ \\
\tb{\scriptsize{6}}\Tt  $(P,\mi{Ts}) := \mi{GenProp}(T,I,C,n)$ \\
\tb{\scriptsize{7}}\Tt  $\mi{Cls} := \mi{Cls} \setminus \s{C}$ \\
\tb{\scriptsize{8}}\Tt  if ($P \equiv 1$) continue \\
\tb{\scriptsize{9}}\Tt  $\mi{Props} := \mi{Props} \cup \s{P}$\} \\
\tb{\scriptsize{10}}\Tt  $\mi{Trcs} := \mi{Trcs} \cup \s{\mi{Ts}}$\} \\
\tb{\scriptsize{11}}\> return($\mi{Props},\mi{Trcs}$)\}  \\
%% \tb{\scriptsize{10}}\Tt  \\
%% \tb{\scriptsize{10}}\Tt  \\
%% \tb{\scriptsize{10}}\Tt  \\
%% \tb{\scriptsize{10}}\Tt  \\

\end{tabbing}}
%\vspace{-20pt}
\caption{Main loop of \ppts}
%\vspace{8pt}
\label{fig:mloop}
%\end{center}
\end{figure}
%% \end{wrapfigure}


==> old_gen_prop.fig.tex <==
%
% GenProp procedure
%
\setlength{\intextsep}{4pt}
\setlength{\textfloatsep}{10pt}
%%\begin{wrapfigure}{l}{1.6in}
\begin{figure}
%\begin{center}
\centering
\small
%\normalsize
%\vspace{5pt}
\parbox{0cm}{\begin{tabbing}
%\begin{tabbing}
aaa\=bb\=cc\= dd\= \kill
$\mi{GenProp}(T,I,C)$\{\\
\tb{\scriptsize{1}}\> $\mi{Trcs} := \emptyset$ \\
\tb{\scriptsize{2}}\> $H_0 := I$; $\abs{H}_0 := \s{H_0}$ \\
\tb{\scriptsize{3}}\> $H_1 := \mi{PQE}(T,I,C)$\\
\tb{\scriptsize{4}}\> if ($H_1 \equiv 1$) return($H_1,\mi{Trcs}$)    \\
\tb{\scriptsize{5}}\> $n := 1$  \\
\tb{\scriptsize{6}}\> while ($\mi{true}$) \{   \\
\tb{\scriptsize{7}}\Tt $\abs{H}_n := \abs{H}_{n-1} \cup \s{H_n}$ \\
\tb{\scriptsize{8}}\Tt $(\mi{ans},\mi{Ts},\abs{H}_n) := \mi{MakeInv}(\abs{H}_n,T)$ \\
\tb{\scriptsize{9}}\Tt if ($\mi{ans} = \mi{succ}$) return($H_n,\mi{Trcs}$) \\
\tb{\scriptsize{10}}\Tt $\mi{Trcs} := \mi{Trcs} \cup \s{\mi{Ts}}$\\
\tb{\scriptsize{11}}\Tt $(H_{n+1},\abs{H}_n) := \mi{PQE}(\abs{H}_n,T)$\\
\tb{\scriptsize{12}}\Tt  $n:=n+1$ \} \\
%% \tb{\scriptsize{1}}\>   \\
%% \tb{\scriptsize{1}}\>   \\
\end{tabbing}}
%\vspace{-20pt}
\caption{\ti{GenProp} procedure}
%\vspace{8pt}
\label{fig:mloop}
%\end{center}
\end{figure}
%% \end{wrapfigure}


==> r0each_diam_known.tex <==
\section{The Case Of Known Reachability Diameter}
\label{sec:rch_diam_on}


==> r1each_diam_unknown.tex <==
\section{The Case Of Unknown Reachability Diameter}
\label{sec:rch_diam_off}


==> s2tr_comp_incons_props.fig.tex <==
%
% RecovProps procedure (structurally complete set of recovery properties)
%
\setlength{\intextsep}{4pt}
\setlength{\textfloatsep}{10pt}
%% \begin{wrapfigure}{l}{1.6in}
\begin{figure}[h]
%\begin{center}
\centering
\small
%\normalsize
%\vspace{5pt}
\parbox{0cm}{\begin{tabbing}
%\begin{tabbing}
aaa\=bb\=cc\= dd\= \kill
$\icp(F)$\{\\
\tb{\scriptsize{1}}\> $\mi{Cls}:=F$    \\
\tb{\scriptsize{2}}\> $\mi{TS} := \emptyset$ \\
\tb{\scriptsize{3}}\> while $(\mi{Cls} \neq \emptyset)$ \{ \\
\tb{\scriptsize{4}}\Tt  $C := \mi{PickCls}(Cls)$ \\
\tb{\scriptsize{5}}\Tt  $\mi{Tst} := \mi{IncPQE}(F,C)$ \\
\tb{\scriptsize{6}}\Tt  $\mi{Cls} := \mi{Cls} \setminus \s{C}$ \\
\tb{\scriptsize{7}}\Tt  if ($\mi{Tst} = \mi{nil}$) continue \\
\tb{\scriptsize{8}}\Tt  $\mi{TS} := \mi{TS} \cup \s{\mi{Tst}}$\} \\
\tb{\scriptsize{9}}\> return($\mi{TS}$)\}  \\
%% \tb{\scriptsize{10}}\Tt  \\
%% \tb{\scriptsize{10}}\Tt  \\
%% \tb{\scriptsize{10}}\Tt  \\
%% \tb{\scriptsize{10}}\Tt  \\

\end{tabbing}}
\vspace{-10pt}
\caption{The \icp procedure}
%\vspace{8pt}
\label{fig:mloop}
%\end{center}
\end{figure}
%% \end{wrapfigure}


==> u1pd_spec.tex <==
\section{Updating Specification}
\label{sec:upd_spec}


